Parallel Batch-Dynamic $k$d-Trees

$k$d-trees are widely used in parallel databases to support efficient neighborhood/similarity queries. Supporting parallel updates to $k$d-trees is therefore an important operation. In this paper, we present BDL-tree, a parallel, batch-dynamic implementation of a $k$d-tree that allows for efficient parallel $k$-NN queries over dynamically changing point sets. BDL-trees consist of a log-structured set of $k$d-trees which can be used to efficiently insert or delete batches of points in parallel with polylogarithmic depth. Specifically, given a BDL-tree with $n$ points, each batch of $B$ updates takes $O(B\log^2{(n+B)})$ amortized work and $O(\log(n+B)\log\log{(n+B)})$ depth (parallel time). We provide an optimized multicore implementation of BDL-trees. Our optimizations include parallel cache-oblivious $k$d-tree construction and parallel bloom filter construction. Our experiments on a 36-core machine with two-way hyper-threading using a variety of synthetic and real-world datasets show that our implementation of BDL-tree achieves a self-relative speedup of up to $34.8\times$ ($28.4\times$ on average) for batch insertions, up to $35.5\times$ ($27.2\times$ on average) for batch deletions, and up to $46.1\times$ ($40.0\times$ on average) for $k$-nearest neighbor queries. In addition, it achieves throughputs of up to 14.5 million updates/second for batch-parallel updates and 6.7 million queries/second for $k$-NN queries. We compare to two baseline $k$d-tree implementations and demonstrate that BDL-trees achieve a good tradeoff between the two baseline options for implementing batch updates.

==> pseudocode/bhl-construct.tex <==
\begin{algorithm}
\caption{Parallel $kd$-Tree Construction}\label{alg:bhl-construct}
\hspace*{\algorithmicindent} \textbf{Input}: Point Set $P$ \\
\hspace*{\algorithmicindent} \textbf{Output}: \kdtree{} over $P$, laid out with a binary-heap layout on a contiguous memory space of size $2|P| - 1$.
\begin{algorithmic}[1]
\Procedure{\buildbhl{}}{$P$}
    \State Allocate $2|P| - 1$ nodes in contiguous memory. The tree nodes will be laid out in this space.
    \State \textsc{\buildbhlrecursive{}($P$, 0, 0)}
\EndProcedure
\Procedure{\buildbhlrecursive{}}{$Q$, $idx$, $c$}
\Statex $idx$: current node index
\Statex $c$: current dimension to split on
\State If we hit the base case $|Q| = 1$, then we construct a leaf node to represent $Q$ at the current index and return.
\State Otherwise, perform a parallel median partition on $Q$ in dimension $c$. Then, place an internal node at the current index to represent this split.
\State Compute $med = |Q|/2$. Then, construct the left and right subtrees in parallel with
\begin{align*}
&\textsc{\buildbhlrecursive{}($Q[:|Q|/2]$, $2idx+1$, $(c+1)\mod{d}$)}\\
&\textsc{\buildbhlrecursive{}($Q[|Q|/2:]$, $2idx+2$, $(c+1)\mod{d}$)}
\end{align*} 
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> pseudocode/single-knn.tex <==
\begin{algorithm}
\caption{Data-Parallel $kd$-Tree $k$-NN}\label{alg:single-knn}
\hspace*{\algorithmicindent} \textbf{Input}: Point Set $P$, int $k$ \\
\hspace*{\algorithmicindent} \textbf{Output}: An array of arrays of the $k$ nearest neighbors of each point in $P$.
\begin{algorithmic}[1]
\Procedure{knn}{$P$}
    \State Allocate a $k$-NN buffer $buf_p$ and Call \textsc{KnnSinglePoint(0, $p$, $k$, $buf_p$)} in parallel over all $p\in P$.
\EndProcedure
\Procedure{knnSinglePoint}{$idx$, $p$, $k$, $buf$}
\State If the current node is a leaf, add all points in the leaf to the $buf_p$ and return.
\State Otherwise, recurse on the child $c$ that $p$ falls within based on the current splitting plane.
\State After the recursive call returns, if $buf_p$ does not yet have $k$ points, simply add all the points in the subtree of $c$'s sibling, $s$.
\State On the other hand, if $buf_p$ has $k$ points, obtain the current radius estimate and call \textsc{knnPrune} on $s$.
\EndProcedure
\Procedure{knnPrune}{$idx$, $p$, $k$, $buf$, $rad$}
\State Call the box centered on $p$ with side lengths $2\cdot rad$ the query box.
\State Compute the box intersection of query box with the bounding box of the current node $idx$.
\State If the boxes are disjoint, return immediately - there are no potential closer neighbors in the subtree.
\State If the query box entirely contains the bounding box, add all the points in the subtree to $buf$ - any of these points could potentially be a closer neighbor.
\State If the boxes otherwise overlap, recurse on the left and right children of $idx$ if it is an internal node. Otherwise, add all of its points to $buf$.
\EndProcedure
\end{algorithmic}
\end{algorithm}

==> sections/methods.tex <==



We will first describe the methods we implemented on the underlying single trees. For insertion and deletion, we implemented two different baselines to compare different tradeoffs. We describe these two baselines in detail below.

Single kdtree Methods
Construction: Both tree types implement coarsened leaves, so that each leaf holds up to a constant number of points (a tunable parameter) rather than a single point.
CO: <how detailed should this be?>
BHL: A simple recursive build routine. Starts from the root node, finds the splitting point, and recurses in parallel over the two children.
Insert
baseline 1: Rebuilds the tree for each insertion. This maintains good balance at the cost of the reconstruction time.
baseline 2: Directly inserts points into the tree without recomputing the split points. This achieves fast insertion times at the cost of potentially skewing the tree.
Delete
baseline 1: Rebuilds the tree for each deletion. This maintains good balance at the cost of the reconstruction time.
baseline 2: Directly deletes points without rebalancing the tree. This achieves fast deletion times at the cost of potentially skewing the tree.
knn: Finds the knn for each point in parallel over all the points. For each individual point, this routine searches through the tree serially, pruning off subtrees based on the current knn radius upper bound and the distance to the bounding box of the subtree.
dual-knn
non-atomic
atomic
array

Log-tree Methods
Insert - <how detailed?>
Construction - construction is implemented by simply calling the insert routine with the point set on an empty tree.
Delete - First, this routine passes the set of points to every individual tree within the logtree and calls the individual tree delete routine on them. Then, it deconstructs and gathers the points from all trees that have been reduced to less than half their original size. Finally, it reinserts all of these points into the structure.
knn - Run knn on all of the individual trees in parallel. This finds the k nearest neighbors for each point within each tree, so we have to find the k nearest neighbors overall afterwards.
knn2 - In parallel over all the points, for each point, run knn sequentially on each of the underlying trees. This avoids the overhead of having to combine results at the end, as we find the true k nearest neighbor for each point in parallel.
knn3 - Run knn on each of the underlying trees sequentially. This implementation makes use of cache-locality as it accesses each tree one at a time, rather than having to continuously switch between trees. It represents a tradeoff between knn and knn2.
dual-knn - Build the query tree and run dual-knn on each underlying tree. In the atomic and array cases (above), we can run in parallel over all of the trees, but we have to reduce the results afterwards as we find the k nearest neighbors of each point within each tree.

